Adversarial Discriminative Domain Adaptation

Adversarial learning methods are a promising approach to training robust deep networks, and can generate complex samples across diverse domains. They also can improve recognition despite the presence of domain shift or dataset bias: several adversarial approaches to unsupervised domain adaptation have recently been introduced, which reduce the difference between the training and test domain distributions and thus improve generalization performance. Prior generative approaches show compelling visualizations, but are not optimal on discriminative tasks and can be limited to smaller shifts. Prior discriminative approaches could handle larger domain shifts, but imposed tied weights on the model and did not exploit a GAN-based loss. We first outline a novel generalized framework for adversarial adaptation, which subsumes recent state-of-the-art approaches as special cases, and we use this generalized view to better relate the prior approaches. We propose a previously unexplored instance of our general framework which combines discriminative modeling, untied weight sharing, and a GAN loss, which we call Adversarial Discriminative Domain Adaptation (ADDA). We show that ADDA is more effective yet considerably simpler than competing domain-adversarial methods, and demonstrate the promise of our approach by exceeding state-of-the-art unsupervised adaptation results on standard cross-domain digit classification tasks and a new more difficult cross-modality object classification task.

==> unified.tex <==
\section{Generalized framework for adversarial domain adaptation}

Existing adversarial adaptation methods all share a basic core idea: representations effective for adaptation are learned via the inclusion of an adversarial loss.
However, these methods vary considerably in the particular details of their instantiations.
Each recent method offers different modeling choices across various factors of variation. 
Some methods seek to minimize the domain distance in a latent discriminatively learned recognition space~\cite{tzeng_iccv15, ganin_jmlr16} while others look to minimize a domain distance in pixel space~\cite{liu_arxiv16}, or perhaps optimizing both spaces simultaneously is best~\cite{donahue_arxiv16}.
Some argue that a single shared representation should be learned~\cite{ganin_jmlr16}, while others claim that only part of the representation should be shared to enable the most effective adaptation~\cite{liu_arxiv16,Yoo2016eccv}.
Then there are more subtle differences in terms of the adversarial learning objective, using either a minimax loss~\cite{goodfellow_nips14, ganin_jmlr16}, an inverted label minimax loss~\cite{goodfellow_nips14}, or a combination confusion loss~\cite{tzeng_iccv15}.
Each subsequent algorithm presents a new setting across these factors, but offers limited motivation or connection to prior work. 
This inherently limits our ability to understand the crucial components of each algorithm and, more importantly, determine how to combine them. 
We unify the existing methods and highlight their variations in Figure~\ref{fig:overview}.

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/overview}
  \caption{Our novel generalized architecture for adversarial domain adaptation.
  Adversarial adaptation methods can be viewed as instantiations of our framework with different choices regarding their properties.}
  \label{fig:overview}
\end{figure}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figs/method}
  \caption{An overview of our proposed Adversarial Discriminative Domain Adaptation (ADDA) approach. We first pre-train a source encoder CNN using labeled source image examples. Then we perform adversarial adaptation by learning a target encoder CNN  such that a discriminator network that sees encoded source and target examples cannot reliably predict their domain label. In our ADDA method, we fix the source encoder while allowing the target encoder to be learned during adversarial adaptation. During testing, target images are mapped with the target encoder to the shared feature space and classified by the source classifier. Note, dashed lines indicate fixed network parameters.  }
  \label{fig:method}
\end{figure*}

All methods learn mappings from source and target inputs to a common high-level feature space. The mappings are instantiated by a base network that can be discriminative, or can include both a discriminative and a generative component. 
Although there are many similarities to generative adversarial networks, we use the more general term ``mapping,'' since many adversarial adaptation methods do not rely on an actual image generator.
The output of this mapping is fed into both a classifier (trained on source) and an adversarial loss that encourages a common feature space. The adversarial loss is minimized when a discriminator network cannot distinguish the domain label of the input. The choices include whether the base mapping is generative or discriminative, whether its weights are tied or untied across domains, and which adversarial loss is used.
We provide a summary of recent adversarial adaptation methods and their choices in Table~\ref{table:properties}.

\begin{table*}
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Method}                       & \textbf{Base model}  & \textbf{Weight sharing}  & \textbf{Adversarial loss} \\
\midrule
Gradient reversal~\cite{ganin_jmlr16} & discriminative       & shared                   & minimax                   \\
Domain confusion~\cite{tzeng_iccv15}  & discriminative       & shared                   & confusion                 \\
CoGAN~\cite{liu_arxiv16}              & generative           & unshared                 & GAN                       \\
ADDA (Ours)                           & discriminative       & unshared                 & GAN                       \\
\bottomrule
\end{tabular}
\caption{
  Overview of adversarial domain adaption methods and their various properties.
  Viewing methods under a unified framework enables us to easily propose a new adaptation method, adversarial discriminative domain adaptation (ADDA).
  }
\label{table:properties}
\end{table*}

\subsection{Base model}
Because unsupervised domain adaptation generally considers discriminative tasks such as classification, previous adaptation methods have generally relied on adapting discriminative models between domains.
With a discriminative base model, input images are mapped into a feature space that is useful for a discriminative task such as image classification.
However, Liu and Tuzel achieve state of the art results on unsupervised MNIST-USPS using two generative adversarial networks~\cite{liu_arxiv16}.
These generative models use random noise as input to generate samples in image space---generally, an intermediate feature of an adversarial discriminator is then used as a feature for training a task-specific classifier.

\subsection{Weight sharing}
Previous adversarial adaptation methods learn a single, symmetric transformation by sharing weights between the source and target networks in order to map images from either domain into a common feature space.
Learning a symmetric transformation reduces the number of parameters in the model.
However, it may make the optimization more poorly conditioned, since the same network must handle images from two separate domains.
Rozantsev et al.~\cite{rozantsev_arxiv16} showed that untied but related weights can lead to effective adaptation in both supervised and unsupervised settings.
As a result, some recent methods have favored untying weights (fully or partially) between the two domains, allowing models to learn parameters for each domain individually.

\subsection{Adversarial loss}
Finally, these adaptation methods employ different adversarial loss functions for their various use cases.
The gradient reversal layer of~\cite{ganin_jmlr16} optimizes the mapping to maximize the discriminator loss directly:
\begin{equation}
\begin{split}
  \min_{M_S,M_T} &\max_D V(D, M_S, M_T) = \\
  &\mathbb{E}_{\mathbf{x}\sim p_S(\mathbf{x})}[\log D(M_S(\mathbf{x}))] \\
  &\quad\quad+ \mathbb{E}_{\mathbf{x}\sim p_T(\mathbf{x})}[\log(1 - D(M_T(\mathbf{x})))]
\end{split}
\end{equation}
where $p_S(\mathbf{x})$ and $p_T(\mathbf{x})$ represent the source and target distributions, respectively, $M_S$ and $M_T$ represent our source and target mappings, which may or may not be identical, and $D$ represents the discriminator.
This optimization corresponds to the true minimax objective for generative adversarial networks.
However, this objective can be problematic, since early on during training the discriminator converges quickly, causing the gradient to vanish.

When training GANs, rather than directly using the minimax loss, it is typical to train the generator with the standard loss function with inverted labels~\cite{goodfellow_nips14}.
This splits the optimization into two independent objectives, one for the generator and one for the discriminator.
The parallel objectives for adversarial adaptation are thus:
\begin{align}
  \begin{split}
    &\max_D\, \mathbb{E}_{\mathbf{x}\sim p_S(\mathbf{x})}[\log D(M_S(\mathbf{x}))] \\
    &\quad\quad+ \mathbb{E}_{\mathbf{x}\sim p_T(\mathbf{x})}[\log(1 - D(M_T(\mathbf{x})))]
  \end{split}\\
  &\max_{M_T}\, \mathbb{E}_{\mathbf{x}\sim p_T(\mathbf{x})}[\log D(M_T(\mathbf{x}))].
\end{align}
This objective has the same fixed-point properties as the minimax loss but provides stronger gradients to the target mapping.
We refer to this modified loss function as the ``GAN loss function'' for the remainder of this paper.
Note that, in this setting, we use independent mappings for source and target, denoted as $M_S$ and $M_T$, and learn only $M_T$ adversarially.
This mimics the GAN setting, where the real image distribution remains fixed, and the generating distribution is learned to match it.

The GAN loss function is the standard choice in the setting where the generator is attempting to mimic another unchanging distribution.
However, in the setting where both distributions are changing, this objective will lead to oscillation---when the mapping converges to its optimum, the discriminator can simply flip the sign of its prediction in response.
Tzeng et al. instead proposed the domain confusion objective, under which the mapping is trained using a cross-entropy loss function against a uniform distribution~\cite{tzeng_iccv15}:
\begin{align}
  \begin{split}
    &\max_D\, \mathbb{E}_{\mathbf{x}\sim p_S(\mathbf{x})}\left[\log D(M_S(\mathbf{x}))\right]\\
    &\quad\quad\quad+ \mathbb{E}_{\mathbf{x}\sim p_T(\mathbf{x})}\left[\log(1 - D(M_T(\mathbf{x})))\right]
  \end{split}\\
  \begin{split}
  &\max_{M_S,M_T} \sum_{d \in \{S,T\}} \mathbb{E}_{\mathbf{x}\sim p_d(\mathbf{x})}\left[\frac{1}{2}\log D(M_d(\mathbf{x}))\right. \\
    &\quad\quad\quad\quad\quad\quad\left.+ \frac{1}{2}\log(1 - D(M_d(\mathbf{x})))\right].
  \end{split}
\end{align}

